CMOSS: A Reliable, Motif-based Columnar Molecular Storage System

The surge in demand for cost-effective, durable long-term archival media, coupled with density limitations of contemporary magnetic media, has resulted in synthetic DNA emerging as a promising new alternative. Despite its benefits, storing data on DNA poses several challenges as the technology used for reading/writing data and achieving random access on DNA are highly error prone. In order to deal with such errors, it is important to design efficient pipelines that can carefully use redundancy to mask errors without amplifying overall cost. In this work, we present Columnar MOlecular Storage System (CMOSS), a novel, end-to-end DNA storage pipeline that can provide error-tolerant data storage at low read/write costs. CMOSS differs from SOTA on three fronts (i) a motif-based, vertical layout in contrast to nucleotide-based horizontal layout used by SOTA, (ii) merged consensus calling and decoding enabled by the vertical layout, and (iii) a flexible, fixed-size, block-based data organization for random access over DNA storage in contrast to the variable-sized, object-based access used by SOTA. Using an in-depth evaluation via simulation studies and real wet-lab experiments, we demonstrate the benefits of various CMOSS design choices. We make the entire pipeline together with the read datasets openly available to the community for faithful reproduction and furthering research.

==> main/6-related-work.tex <==
\section{Related Work}

Biologists have long demonstrated the ability to store data in DNA~\cite{clelland}. However, using DNA as a ``large-scale'' data storage media is an entirely new area of research that has become possible only recently, thanks to advances in sequencing and synthesis technologies. Almost all prior work on DNA data storage has focused on developing encoding techniques for mapping binary files to oligos. We only present an overview of a few key related publications in this section. A comprehensive survey of approaches can be found here~\cite{heinis2019survey}. 

Pioneering work by Church et al.~\cite{church-synthesis} was the first to prove the viability of DNA as a large-scale digital storage medium. Using a simple coding scheme that maps a 0 bit in the input stream to an A or C and a 1 bit to G or T, they stored a HTML file of 0.65MB. However, due to errors in sequencing and synthesis procedures, data retrieval was not fully automated and required manual intervention. Following this, Goldman et al. proposed a variable-length coding scheme that improves storage density by compressing and transforming data into an intermediate base-3 representation~\cite{goldman2013towards}. Using this procedure, they stored 739KB of digital data and showed that encoding/decoding of data can be done automated despite errors.

Follow up work investigated error-correction techniques that can provide full recovery while substantially improving storage density. Bornholt et al. optimized Goldman et al.'s strategy by implementing simple XOR-based redundancy~\cite{dna-archive}. Grass et al.~\cite{grass2015robust} proposed an error-correcting scheme that used concatenation codes with Reed Solomon codes as both inner and outer codes to store 83KB of data. 
Blawat et al.~\cite{Blawat-fec} study the error properties of DNA storage based on the results from the first study by Church et al. Using a forward error-correction code customized to the DNA erasure channel, they stored 22MB of data. Organick et al.~\cite{organick2018random} propose a new concatenation code with Reed-Solomon as the outer code and the differential code from Goldman et al. as the inner code. Using this new code, they stored and recovered 200MB of data. We compared CMOSS with several of these methods in Section~\ref{sec:evaluation}.
